Status substitution and conspicuous consumption

This paper adapts ideas from social identity theory to set out a new framework for modelling conspicuous consumption. Agents derive utility from their consumption of a status good and from belonging to an identity group with high status good consumption. Importantly, these two sources of utility are substitutes. Agents also feel pressure to conform with their neighbours in a network. This framework can rationalise a set of seemingly conflicting stylised facts about conspicuous consumption that are currently explained by different families of models. In addition, our model delivers new testable predictions regarding the effect of network structure and income inequality on conspicuous consumption.

==> setup.tex <==
\RequirePackage{etex} 
% bibliography packages ---------------------------------
\usepackage{natbib}
% maths packages ----------------------------------------
\usepackage{amsmath, amsthm, amssymb, amsfonts}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
% images packages ---------------------------------------		
\usepackage{graphicx}
%\usepackage{sidecap}
\usepackage{subcaption}
\renewcommand\thesubfigure{\arabic{subfigure}} % Number subfigures (i.e. 1,2,3... rather than a,b,c...
\usepackage{caption}
\usepackage{comment}
\usepackage{float}
% tikz image packages -----------------------------------		
\usepackage{tikz}
\usepackage{pgf, pgfplots}
\usepackage{tikz-network}
%\usepackage{tkz-graph}
%\usetikzlibrary{graphs, graphs.standard, quotes}% quotes library is for the [""] edges
\pgfplotsset{compat=1.17} 
\usepackage{xcolor}
% tikz libraries ----------------------------------------	
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{decorations.markings}
% other packages ----------------------------------------
\usepackage{setspace}
\usepackage{fullpage}
\usepackage{pdfpages}
\usepackage{import}
\usepackage{rotating}
\usepackage{hyperref}
\usepackage{cleveref} % clever referencing package
\usepackage{minitoc}
\usepackage{algpseudocode} %algorithm environment
% other settings ----------------------------------------
% this sets the border colour and background colour (respectively) of the fbox. We put an fbox around the network images to make them easier to control. Toggle the border colour between black and white to show/hide the borders
\renewcommand\fbox{\fcolorbox{white}{white}}
% THEOREMS ----------------------------------------------
\newtheorem{thm}{Theorem}       
\newtheorem*{thm*}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem*{prop*}{Proposition} 
\newtheorem{cor}{Corollary}     
\newtheorem{lem}{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{defn}{Definition}
\newtheorem{rem}{Remark} 
\newtheorem*{rem*}{Remark} 
\newtheorem{ex}{Example} 
\newtheorem*{ex*}{Example} 
\newtheorem{ass}{Assumption}
\newtheorem{res}{Result}
\newtheorem{conj}{Conjecture}

\newtheorem{innercustomprop}{Proposition}
\newenvironment{customprop}[1]
  {\renewcommand\theinnercustomprop{#1}\innercustomprop}
  {\endinnercustomprop}
% commenting ------------------------------------------
\usepackage{comment}
\definecolor{green}{HTML}{51A351}
\definecolor{blue}{HTML}{2F96b4}
\definecolor{gray}{HTML}{BCBCBC}

% Maths operators ------------------------------------
\DeclareMathOperator*{\argmax}{arg\max}
\DeclareMathOperator*{\argmin}{arg\min}
% Other user defined functions -----------------------
\newcommand{\B}{\mathcal{B}}
\renewcommand{\d}{\mathrm{d}}
%\newcommand{\deg}{\mathrm{deg}}
\newcommand{\peel}[2]{\mathrm{Peel}_{#1}\left({#2}\right)}
% A hack to get just month and year in the date
\newcommand{\monthyeardate}{\ifcase \month \or January\or February\or March\or April\or May \or June\or July\or August\or September\or October\or November\or December\fi, \number \year}
% Page setup -----------------------------------------
\onehalfspacing
% Set watermark
%\usepackage{draftwatermark}
%\SetWatermarkText{Confidential Draft}
%\SetWatermarkScale{5}
%\SetWatermarkAngle{55}
%\DraftwatermarkOptions{color={[gray]{0.85}}}
